EXCLAIM: An Explainable Cross-Modal Agentic System for Misinformation Detection with Hierarchical Retrieval

Misinformation continues to pose a significant challenge in today's information ecosystem, profoundly shaping public perception and behavior. Among its various manifestations, Out-of-Context (OOC) misinformation is particularly obscure, as it distorts meaning by pairing authentic images with misleading textual narratives. Existing methods for detecting OOC misinformation predominantly rely on coarse-grained similarity metrics between image-text pairs, which often fail to capture subtle inconsistencies or provide meaningful explainability. While multi-modal large language models (MLLMs) demonstrate remarkable capabilities in visual reasoning and explanation generation, they have not yet demonstrated the capacity to address complex, fine-grained, and cross-modal distinctions necessary for robust OOC detection. To overcome these limitations, we introduce EXCLAIM, a retrieval-based framework designed to leverage external knowledge through multi-granularity index of multi-modal events and entities. Our approach integrates multi-granularity contextual analysis with a multi-agent reasoning architecture to systematically evaluate the consistency and integrity of multi-modal news content. Comprehensive experiments validate the effectiveness and resilience of EXCLAIM, demonstrating its ability to detect OOC misinformation with 4.3% higher accuracy compared to state-of-the-art approaches, while offering explainable and actionable insights.

==> secs/05_discussion.tex <==
%!TEX root = ../main.tex
\subsection{Discussion}

\subsubsection{Why not Open-source Model?}

\begin{table*}[t!]
\centering
\caption{Accuracy comparison (\%) between the GPT-4o and LLava Models.}
\label{table: discussion_llava}
\begin{tabular}{lcccc}
\toprule
\textbf{} & \textbf{GPT-4o-Latest} & \textbf{GPT-4o-mini} & \textbf{LLaVA-13B} & \textbf{LLaVA-7B}\\
\hline
\textbf{Accuracy}           & \cellcolor{lightgray}91.7\%         & 84.6\%          & 56.2\%     &   43.8\%  \\
\hline
\end{tabular}
\end{table*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figs/Figure_4_error.pdf}
    \caption{Error Distribution of GPT-4o and LLaVA Models on Different Type OOC Misinformation.}
    \label{fig:disucssion_errors}
\end{figure*}

In this section, we discuss the impact of replacing the base model in our multi-agent system with open-source alternatives. To better understand the implications of such a change, we conducted a detailed analysis using the four data types provided by the NewsCLIPpings dataset.  The NewsCLIPpings dataset defines three primary types of image-text mismatches. Semantics Matching involves pairing images with captions that align in general content but differ in specific entities or events. This is split into two subtypes: \textbf{\textit{Text-Image}}, which retrieves images based on overall visual-textual similarity, and \textbf{\textit{Text-Text}}, where a semantically similar caption is first found, and the image from that caption is then mismatched with the original text. \textbf{\textit{Person Matching}} focuses on cases where the correct individual is depicted, but the person is placed in a misleading or unrelated context. Finally, \textbf{\textit{Scene Matching}} mislabels the broader setting or event, ensuring the environment looks similar but describes a different situation, excluding any references to individuals. For our evaluation, we maintained an equal distribution of 1,000 samples, with 250 examples from each category, to ensure a balanced and comprehensive assessment of model performance across these different misinformation scenarios.


Table~\ref{table: discussion_llava} shows a clear performance gap between open-source models like LLaVA 1.5~\citep{liu2023llava} and closed-source counterparts. Despite using the CLIP-ViT-L-336px architecture, LLaVA-7B and LLaVA-13B struggled with \textit{Person Matching} and \textit{Scene Matching} tasks, tasks requiring precise visual-textual alignment. Their smaller parameter sizes (7B and 13B) and shorter context windows limited their ability to process complex scenes. Prompt engineering yielded minimal improvements, emphasizing the architectural constraints in handling advanced multi-modal reasoning.

In contrast, closed-source GPT-4o models excelled across all OOC misinformation categories, as shown in Figure~\ref{fig:disucssion_errors}. Their larger parameter sizes and extended context windows allowed for better handling of intricate cross-modal relationships, especially in \textit{Scene Matching}, which requires deep contextual understanding. Additionally, the ease of deployment and regular updates of commercial models offer further advantages. Using state-of-the-art closed-source models improves the robustness of our misinformation detection system while avoiding the complexities of local deployment. Continuous updates ensure that our \textbf{\texttt{EXCLAIM}} framework remains at the forefront of multi-modal misinformation detection.

% Conversely, the closed-source GPT-4o models exhibited superior performance across all data types. Their larger parameter sizes and extended context windows enabled them to handle complex cross-modal relationships, particularly in \textit{Scene Matching} tasks, which demand a deep understanding of contextual shifts between text and images. This advantage is further amplified by the ease of deployment and continuous updates available with commercial models. By utilizing SOTA closed-source models, we can not only build a more robust and efficient misinformation detection system but also avoid the complexities of local deployment. Additionally, as commercial models are frequently updated, each new iteration enhances the performance of our \textbf{\texttt{EXCLAIM}} framework, ensuring that it remains at the forefront of multimodal misinformation detection.

\subsubsection{Explainability Analysis}

\begin{table*}[t!]
\centering
\caption{Average rankings of four methods for logic and explanation (human and GPT-4o evaluations). The best results for each test data are highlighted in bold.}
\label{table: discussion expla}
\begin{tabular}{lcccc}
\toprule
  \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Human}} & \multicolumn{2}{c}{\textbf{GPT-4o}} \\ 
 \cmidrule{2-5} & Logic & Explanation & Logic & Explanation \\ \midrule
LLaVA (few-shot)&  3.40& 3.55 &3.50  &3.55  \\
GPT-4o (few-shot)& 2.45 & 2.33  & 2.15 & 1.73  \\
\textbf{\texttt{EXCLAIM}} (LLaVA) & 2.90 & 3.03 & 3.08 & 3.40 \\
\textbf{\texttt{EXCLAIM}} (GPT-4o) & \cellcolor{lightgray}\textbf{1.25} & \cellcolor{lightgray}\textbf{1.10} & \cellcolor{lightgray}\textbf{1.28} & \cellcolor{lightgray}\textbf{1.33} \\ \hline
\end{tabular}
\end{table*}
To assess the quality of explanations generated by the \textbf{\texttt{EXCLAIM}} framework, we conducted evaluations using both human evaluation and GPT-4o evaluation. Our comparison encompassed four configurations: two models (LLaVA-1.5-13B and GPT-4o-Latest) implemented within our \textbf{\texttt{EXCLAIM}} framework, and the same two models applied directly in a few-shot setting. For each of the 40 randomly selected test samples, both human evaluators and GPT-4o ranked the explanations generated by the four base models according to two criteria: \textbf{logical consistency (Logic)} and \textbf{explanatory quality (Explanation)}. Each model was assigned a rank from 1 (best) to 4 (worst) for each test case, and the average ranking across all samples was calculated for both logic and explanation.

As shown in Table~\ref{table: discussion expla}, \textbf{\texttt{EXCLAIM}} (GPT-4o) demonstrated superior performance across all evaluation metrics, achieving the lowest average rankings in both human and GPT-4o assessments. Specifically, human evaluators assigned \textbf{\texttt{EXCLAIM}} (GPT-4o) average rankings of 1.25 for logic and 1.10 for explanation, while GPT-4o evaluation yielded similar results with rankings of 1.28 and 1.33, respectively. These consistent results across different evaluation methods underscore the framework's robust capability in generating logically sound and clear explanations.

Interestingly, we observed that the few-shot GPT-4o baseline performed notably better than the few-shot LLaVA-1.5, suggesting the inherent strength of GPT-4o in handling OOC news detection. However, the \textbf{\texttt{EXCLAIM}} framework substantially enhanced GPT-4o's performance, as evidenced by the improvement from few-shot GPT-4o (2.45, 2.33 for human evaluation) to \textbf{\texttt{EXCLAIM}} (GPT-4o) (1.25, 1.10). This improvement validates the effectiveness of our framework in refining both logical reasoning and explanation generation capabilities.

A notable observation emerged when comparing human and GPT-4o evaluations of the few-shot GPT-4o method. The GPT-4o evaluator assigned more favorable scores (2.15, 1.73) compared to human evaluators (2.45, 2.33), suggesting a potential bias in GPT-4o's self-assessment. This finding aligns with previous research~\cite{wang2023large,zheng2023judging} on large language models' tendency toward self-favorability in evaluation tasks.

\subsection{Error Analysis Across Different Misinformation Categories}
\label{ssse:category_ana}
To provide a more comprehensive understanding of \textbf{\texttt{EXCLAIM}}'s performance characteristics, we conducted a detailed analysis of error cases across different categories in the NewsCLIPpings dataset. Table \ref{tab:error_distribution} presents the distribution of errors across the four primary categories: \textbf{\textit{Text-Image}}, \textbf{\textit{Text-Text}}, \textbf{\textit{Scene-Matching}}, and \textbf{\textit{Person-Matching}}.

\begin{table*}[h]
\centering
\caption{Distribution of Error Cases Across Different Categories in NewsCLIPpings Test Dataset.}
\begin{tabular}{lccc}
\toprule
\textbf{Category} & \textbf{Error Count} & \textbf{Error Rate (\%)} & \textbf{Primary Error Patterns} \\
\midrule
Text-Image & 177 & 33.40\% & Semantic similarity confusion \\
Person-Matching & 174 & 32.83\% & Contextual misalignment \\
Scene-Matching & 106 & 20.00\% & Environmental ambiguity \\
Text-Text & 73 & 13.77\% & Narrative consistency issues \\
\hline
Total & 530 & 100.00\% & - \\
\hline
\end{tabular}
\label{tab:error_distribution}
\end{table*}

Our analysis reveals several noteworthy patterns in \textbf{\texttt{EXCLAIM}}'s error distribution. Text-Image mismatches constitute the largest proportion of errors (33.40\%), suggesting that the framework faces the greatest challenges in cases where semantic similarities between images and text are subtly misaligned. This is closely followed by Person-Matching errors (32.83\%), indicating that distinguishing individuals in different contexts remains a significant challenge despite our multi-agent approach.

Scene-Matching errors account for 20.00\% of the total errors, primarily occurring in cases where environmental elements share visual similarities but represent different events or contexts. The lowest error rate was observed in Text-Text matching (13.77\%), suggesting that \textbf{\texttt{EXCLAIM}} performs relatively well in detecting inconsistencies when dealing with purely textual semantic relationships.

These findings suggest potential areas for future improvement:

\begin{enumerate}
    \item \textbf{Enhanced semantic reasoning capabilities:} Improving the system's ability to detect subtle semantic misalignments between images and text, particularly in cases where surface-level similarities mask contextual inconsistencies.
    
    \item \textbf{Refined person-context association:} Strengthening the framework's capability to accurately track and verify person-specific contextual information across different temporal and spatial settings.
    
    \item \textbf{Advanced scene understanding:} Developing more sophisticated mechanisms for distinguishing between visually similar but contextually different environments and events.
    
    \item \textbf{Improved narrative consistency checking:} Enhancing the system's ability to verify and validate textual narrative consistency across different sources and contexts.
\end{enumerate}

This error distribution analysis provides valuable insights for future iterations of the \textbf{\texttt{EXCLAIM}} framework and highlights specific areas where additional attention could yield significant improvements in overall system performance.
